Equilibrium and traveling-wave solutions of plane Couette flow

We present ten new equilibrium solutions to plane Couette flow in small periodic cells at low Reynolds number (Re) and two new traveling-wave solutions. The solutions are continued under changes of Re and spanwise period. We provide a partial classification of the isotropy groups of plane Couette flow and show which kinds of solutions are allowed by each isotropy group. We find two complementary visualizations particularly revealing. Suitably chosen sections of their 3D-physical space velocity fields are helpful in developing physical intuition about coherent structures observed in low Re turbulence. Projections of these solutions and their unstable manifolds from their infinite-dimensional state space onto suitably chosen 2- or 3-dimensional subspaces reveal their interrelations and the role they play in organizing turbulence in wall-bounded shear flows.

==> aspect.tex <==
% aspect.tex
% $Author: predrag $ $Date: 2008-08-22 12:43:04 -0400 (Fri, 22 Aug 2008) $

%\section{Bifurcations under spanwise variation of $L_z$}
%\label{s:aspect}

\begin{figure}
\centering
{\small (a)} \includegraphics[width=0.45\textwidth]{bifur_Lz_double}%
{\small (b)} \includegraphics[width=0.45\textwidth]{bifur_gamma}%
   \caption[Bifurcations of \eqva\ under change in spanwise length.]{
Dissipation rate $D$ of \eqva\ for family of cells $\bCell(L_z) =
[2\upi/1.14,2,L_z]$ as function of (a) the spanwise cell width $L_z$
(b) wavenumber $\gamma = 2 \upi/L_z$.
The vertical dashed lines represent the \bNarrow\ cell at
$L_z=2.51$, $\gamma = 2.5$, and the vertical dotted line marks the
\bHKW\ cell at $L_z=3.76$, $\gamma = 1.67$.
\sLB\ \tLB,  \sUB\ \tUB,
\sNNB\ \tNNB,   \sNB\ \tNB,   \sEQfive\ \tEQfive,
\sEQsev\ \tEQsev\,   \sEQnine\ \tEQnine,
\sEQten\ \tEQten,   \sEQelev\ \tEQelev.
The repeated solution
curves at doubled values of $L_z$ indicate solutions of fundamental
periodicity $L_z$ embedded in a cells with spanwise length $2 L_z$.
(see \reffig{f:HKW-eqva}).
\Eqva\  \sEQsix\ \tEQsix,  \sEQeight\ \tEQeight\ do not exist at
$\Reynolds=400$.
We did not attempt to continue \tTWone, \tTWDone, or \tTWthree.
}
\label{f:spanwise-eqva}
\end{figure}
In this section we examine changes in solutions under variation in spanwise
periodicity. In particular, we are interested in connecting the solutions for
\bNarrow\ discussed in \refsect{s:eqba}, to the wider \bHKW\ cell of \cite{HaKiWa95},
which empirically exhibits sustained turbulence
at $\Reynolds = 400$.
\refFig{f:spanwise-eqva} shows dissipation as a function of $L_z$. Of the
\eqva\ discussed above, only \tNB, \tEQsev, and \tEQnine\ could be continued
from \bNarrow\ to \bHKW\ at $\Reynolds = 400$. The other
\eqva\ terminate in saddle-node bifurcations, or bifurcate into pairs
of \reqva\ in pitchfork bifurcations.
\tLB\ and \tUB\ exist in \bHKW\
as spanwise doubled $2 \times \tLB$ and  $2 \times \tUB$ in $z$.
We insert 2 copies of the \tLB\,/\,\tUB\ solution
for $\bNarrow$, with $L_z \approx 2.51$, into a cell
with $L_z \approx 5.02$, and then continue these solutions down to
the  $\bHKW$ width $L_z = 3.76$.

\refFig{f:HKW-eqva} shows 3D velocity fields
for all of these {\eqva} in \bHKW: \tNB, \tEQsev, and \tEQnine\ and the
spanwise doubled $2 \times \tLB$ and $2 \times \tUB$.
Their properties are listed in \reftab{t:eqbtableHKW}.

\begin{figure}
\centering
\includegraphics[width=0.35\textwidth]{uNB_HKW_R400} \hskip -28ex \tNB \hskip 22ex
\includegraphics[width=0.30\textwidth]{uEQ7HKWbox} \hskip -27ex \tEQsev \hskip 24ex
\includegraphics[width=0.30\textwidth]{uEQ9HKWbox} \hskip -27ex \tEQnine \hskip 24ex ~\\
\includegraphics[width=0.35\textwidth]{u2LB_HKW_R400} \hskip -30ex $2 \times \tLB$ \hskip 15ex
\includegraphics[width=0.35\textwidth]{u2UB_HKW_R400} \hskip -30ex $2 \times \tUB$ \hskip 15ex ~
\caption[Physical space plots of HKW cell \eqva.]{
 Equilibria in the \bHKW\ cell of \cite{HaKiWa95}, $\Reynolds = 400$.
 \tNB, \tEQsev, \tEQnine, and the spanwise-doubled \eqv\ solutions
 $2 \times \tLB$ and $2 \times \tUB$.}
\label{f:HKW-eqva}
\end{figure}


The low dissipation values of the \bHKW\ {\eqva}
\reffig{f:IvD-W03}\,(b)
suggest that they
are not involved in turbulent dynamics, except perhaps as gatekeepers to
the laminar equilibrium. We
suspect that yet undiscovered {\eqva}, 
or already known \po\ solutions \citep{GHC08a}
do play a key role in organizing turbulent dynamics.

However, unlike the \bNarrow\ cell, we were not able to find any {\eqva}
for \bHKW\ cell from initial guesses sampled from long-time
turbulent trajectories within the $S$-invariant subspace. This is curious,
contrasted to our success in finding {\eqva} from such
guesses in \bNarrow, and suggests that the aspect ratios of the
\bHKW\ cell are the most incommesurate (fit the intrinsic widths of rolls
least well) compared to spanwise-infinite plane Couette's
roll and streak scales apparent in the simulation of \reffig{f:bigbox}.

In the \bHKW\ cell \tNB\ is extremely unstable, with a 39 dimensional
unstable manifold. In physical space it has 4 distinct streaks, see \reffig{f:HKW-eqva}.
Owing to its near $\trHalf{z}$ symmetry, many of its eigenvalues appear
in sets of two nearly identical complex pairs.


\begin{table}
\centering
\begin{tabular}{l|lllccc}
          & ~~$\Norm{\cdot}$   & ~~$E$
          & ~$D$ & $H$ & $\dim W^u$ & $\dim W^u_{H}$  \\ % & acc.\\
\hline
mean          & 0.40   & 0.15   & 3.0      &           &    &     \\ % &   \\
\tLM          & 0      & 0.1667 & 1        & $\GPCF$   & ~0 & ~0   \\ % & 0\\
$2\times$\tLB & 0.2458 & 0.1112 & 1.8122   &\PCedit{$S \times \{e, \tau_{z}\}$}& ~5 & ~0   \\ % & ?\\
$2\times$\tUB & 0.3202 & 0.0905 & 2.4842   &\PCedit{$S \times \{e, \tau_{z}\}$}& ~6 & ~0   \\ % & ? \\
\tNB          & 0.2853 & 0.0992 & 2.4625   & $S$       & 40 & 13  \\ % & ?\\
\tEQsev       & 0.1261 & 0.1433 & 1.3630   & \PCedit{$S \times \{e, \tau_{xz}\}$}& ~6 & ~2   \\ % & ? \\
\tEQnine      & 0.3159 & 0.1175 & 2.0900   & $\{e, \sigma_{xz}\}$  & 11 & 0  \\ % & ?
\end{tabular}
\label{t:eqbtableHKW}
\caption[Properties of invariant solutions.]{
Properties of \eqv\ and \reqv\ solutions for \bHKW\ cell, $\Reynolds=400$,
defined as in \reftab{t:eqbtable5}. See also \reffig{f:IvD-W03}\,(b).
}
\end{table}


==> bifurRe.tex <==
% bifurRe.tex
% $Author: predrag $ $Date: 2008-08-22 12:43:04 -0400 (Fri, 22 Aug 2008) $

% \section{Bifurcations under variation of \Reynolds}
% \label{s:bifurRe}

\begin{figure}
\centering
{\small (a)}\includegraphics[width=0.45\textwidth]{D_bNarrow_all}%
~~{\small (b)}\includegraphics[width=0.47\textwidth]{D_bNarrow_all_detail}
\caption[Bifurcations of (relative) equilibria under variation of \Reynolds.]{
(a) Dissipation rate as a function of Reynolds number for all \eqva\ in
in the $\bNarrow$ cell.
(b) Detail of (a).
\sLB\ \tLB, \sUB\ \tUB, \sNNB\ \tNNB, \sNB\ \tNB,
\sEQfive\ \tEQfive, \sEQsix\ \tEQsix, \sEQsev\ \tEQsev, \sEQeight\ \tEQeight,
\sEQnine\ \tEQnine, \sEQten\ \tEQten, \sEQelev\ \tEQelev,
\sTWone\ \tTWone, and \sTWthree\ \tTWthree.
}
\label{f:bifurRe}
\end{figure}

The relations between the equilibrium and traveling-wave solutions can be clarified
by tracking their properties under changes in \Reynolds\ and cell size variations.
\refFig{f:bifurRe} shows a bifurcation diagram for \eqva\ and \reqva\ in
the $\bNarrow$ cell, with dissipation rate $D$ plotted against $\Re$ as
the bifurcation parameter. A number of independent solution curves are shown
in superposition.
This is a 2-dimensional projection from the $\infty$-dimensional
\statesp, thus,
unless noted otherwise,
the apparent intersections of the solution
curves do not represent bifurcations; rather, each curve is a family of
solutions with an upper and lower branch, beginning with a saddle-node
bifurcation at a critical Reynolds number.

The first saddle-node bifurcation gives birth to the Nagata lower branch
\tLB\ and upper branch \tUB\ \eqva, at $\Re \approx 218.5$.
\tLB\ has a single $S$-invariant unstable eigenvalue
(and additional subharmonic instabilities that break the
$S$-invariance of \tLB).
Shortly after bifurcation, \tUB\ has an unstable complex eigenvalue pair within the
$S$-invariant subspace and two unstable real eigenvalues leading out of that space.
As indicated by
the gentle slopes of their bifurcation curves, the \cite{N90} solutions are
robust with respect to Reynolds number. The lower branch solution has been
continued past $\Re =10,000$ and has a single unstable eigenvalue throughout
this range \citep{WGW07}.

\tNNB\ and \tNB\ were discovered in independent Newton searches and subsequently
found by continuation to be lower and upper branches of a saddle-node
bifurcation occurring at $\Reynolds \approx 364$. \tNNB\ has a leading unstable
complex eigeinvalue pair within the $S$-invariant subspace. Its remaining two unstable
eigen-directions are nearly marginal and lead out of this space.

\tEQsix\ was found by continuing \tEQfive\ backwards in $\Reynolds$ around the
bifurcation point at $\Reynolds \approx 326$. We were not able to continue \tEQsix\
past $\Reynolds=330$. Just beyond  $\Reynolds = 330$
the dynamics in this region appears to be roughly periodic, suggesting that \tEQsix\
undergoes a supercritical Hopf bifurcation here. At $\Reynolds \approx 348$,
\tEQten~/~\tEQelev\ are born in a saddle node bifurcation, similar in character
to the \tLB\ / \tUB\ bifurcation.

\refFig{f:bifurRe}{\textit(b)} shows several symmetry-breaking bifurcations.
At $\Reynolds \approx 250$, \tTWone\ bifurcates from \tLB\ in a
subcritical pitchfork as an $s_2$-symmetric, $s_1,s_3$-antisymmetric
eigenfunction of \tLB\ becomes unstable, resulting in a
spanwise-moving \reqv. At $\Reynolds \approx 370$, the $\tEQnine$
\eqv\ bifurcates off \tNB\ along an $\sigma_{xz}$-symmetric,
$s_1,s_2$-antisymmetric eigenfunction of \tNB.
Since $\sigma_{xz}$ symmetry fixes
phase in both $x$ and $z$,  this solution bifurcates off \tNB\ as an
equilibrium rather than a traveling wave.


==> figs/epscolor2bw <==
#!/usr/bin/perl

# Convert color EPS to BW

while (<>) {
  s/\%\%BeginProlog\n/\%\%Prolog\n\/setrgbcolor \{0.11 mul 3 1 roll 0.59 mul 3 1 roll 0.30 mul add add setgray\} def\n/;
  print;
}


==> flotsam.tex <==
% flotsam.tex of stuff exiled from n00bs.tex
% $Author: predrag $ $Date: 2009-05-01 17:28:43 -0400 (Fri, 01 May 2009) $

% enter most recent flotsam to the top of this file:
% Predrag                                           25 Jul 2007
%     gibson/steady/flotsam.tex poetry banished from steady.tex
%     now definitely moved to Halcrow thesis
% Predrag started JH thesis collection here         13 Sep 2005



% \section*{Flotsam}

\medskip
\noindent
{\bf PC:} add paragraph on pipe \reqva\ and absence
 of \eqva.
 The laminar state is also believed to be linearly stable for
 the Hagen-Poiseuille (pipe) flow for all \Reynolds.  However,
 \eqva\ other than the laminar state have not been computed.
     According to my understanding, there cannot be any. Pipe has
 $SO(2)\times O(2)$ symmetry, so there are solutions with one of the
 shifts =0, but not both the streamwise and the cylindrical shifts
 =0.

 Pass over in silence lower-dimensional models.


\medskip

\noindent
{\bf PC:}
    please enter into bibtex/halcow.bib the relevant ones from this
    list

           (7) G. Kawahara,

              Laminarization of minimal plane Couette flow:
              Going beyond the basin of attraction of turbulence,
              Phys. Fluids, 17-4 (2005), 041702-1-041702-4.

            (9) G. Kawahara and S. Kida,
              Elementary coherent structures in turbulent flows,
              Parity, 20-12 (2005).

           (10) \cite{VKK05}
              Periodic motion representing isotropic turbulence,
              Fluid Dynamics Research, 38 (2006), 19-46.

           (11) G. Kawahara, S. Kida and L. van Veen,
              Unstable periodic motion in turbulent flows,
              Nonlinear Process in Geophysics, 13 (2006), 499-507.

\noindent
{\bf JH:}
    Did not enter (7), (10), (11),
    didn't seem relevant to this particular paper.
    Could not find (9) checked chaosbook library, google scholar,
    arxiv and ebsco is it japanese?



\medskip

\subsection*{On $2D$ Disturbances}

\JH{This section could probably go if we need to cut down on space}
    \PC{merge this with Wally's derivation, in the report in
        halcrow/blog/}
If we force the \NSe\ to be streamwise independent (\ie set $\partial_x = 0$), the
spanwise and wall-normal velocities act independently
of the streamwise velocity\cite{W95a}:
\bea
\partial_t v + v \partial_y v + w \partial_z v &=& -\partial_y p + \nu \nabla^2 v \\
\partial_t w + v \partial_y w + w \partial_z w &=& -\partial_z p + \nu \nabla^2 w \\
\partial_y v + \partial_z w &=& 0
\eea
The streamwise velocity is now governed by a linear equation, forced by $v$ and $w$ :
\beq
\partial_t u + v \partial_y u + w \partial_z u = \nu \nabla^2 u
\,.
\eeq

Without the streamwise velocity, there is no energy input in
the $(v,w)$ system. So, the viscosity will eventually damp out
any disturbances.  More rigorously, the rate of change of the
disturbance kinetic energy $E = \frac{1}{2} \int u_i'^2 dx$, is
given by the Reynolds-Orr energy equation \citep{DR04},
\beq
\frac{dE}{dt} = - \int u_j' u_i' D_{ij} + R^{-1} (\partial_j u'_i)^2 dx
\,,
\ee{eq:ReynoldsOrrEnergy}
where $D_{ij}$ is called the `rate of strain tensor' of the base flow
\beq
D_{ij} = \frac{1}{2}(\partial_j U_i + \partial_i U_j)
\,.
\eeq
In the case of streamwise independent flow, since $(v,w)$ is
decoupled from $u$, we can drop the streamwise parts.  Since $V
= W = 0$, $D_{ij} = 0$.  Therefore the integrand in equation
\ref{eq:ReynoldsOrrEnergy} is strictly non-negative. So we can
rule out any periodic solutions. An \eqva\ would have to
satisfy $\partial_j u_i = 0$. Since we have no-slip boundary
conditions, this clearly implies that the only steady state is
$v = w = 0$. It is demonstrated in \cite{W95a,W97}
that low-amplitude, streamwise-independent rolls produce strong
streaks which do have a strong streamwise instability (and thus
the SSP turns).


\medskip
{\bf  PC:}
I use
   $[L_x,2,L_z]$ convention rather than $(\alpha,\gamma)$,
    because at  $\Reynolds = 400$ the roll
   spanwise  diameter is roughly 1.5-2, and the spanwise aspect ratio
   $L_z$/(roll width) counts how many roll pairs (transverse wavelengths)
   we fit.

\medskip
{\bf JFG comments to PC cell size discussion: }
I hear what you're saying about $L_x$ and $L_z$
not being parameters, but I think this is a better way of saying it. Particularly,
you don't want to say that $L_y$ sets the length scale, wall velocity the time
scale, leaving $\Reynolds$ as the only parameter. Physical length and time have
already been non-dimensionalized away into the Reynolds number. The size of the rolls
is not simply given by $L_y$. At higher Reynolds, the rolls gets smaller than $L_y$.
As best we know, the rolls size is determined by the wall units, which are determined
by the wall shear rate and cannot be given a priori from the flow parameters (as far
as we know). We don't want to get into this here.

\medskip
A further important detail that can make it
difficult to compare numerical results (mostly glossed over
in the literature) is the choice of an external pressure or
mean-velocity constraint that governs the evolution of the mean
flow. As explained in \refsect{s:review}, we hold the spatial mean
of the pressure gradient fixed at zero and let the mean velocity
vary independently.
    \PC{
    pressure does not affect steady solutions, right? Maybe
        can drop this remark. }

\medskip
\tEQsix\ and
\tEQeight, the upper-branch partners of \tEQfive\ and \tEQsev, were found by
continuing the latter in \Reynolds\ around their bifurcation points,
using a quadratic extrapolation
and the Newton-hookstep descent.

\medskip
It bifurcates from \tLB\ in a subcritical
pitchfork, and is associated
with the stabilization of an eigenfunction which is symmetric with
respect to $s_2$, but antisymmetric with respect to $s_1$ and $s_3$.
Thus, the \reqv\ retains $s_2$ symmetry according to the
Equivariant Branching Lemma \citep{golubitsky2002sp}.
   \JH{
The EBL doesn't exactly apply as is (it requires things like
the group acting absolutely irreducibly on the space and the fixed subspace
of the bifurcated subgroup to be one dimensional), but I think an argument
can be made looking a 2d slice of the space in a neighborhood of uLB near
bifurcation(one direction being the bifurcating eigenfunction,
the other some fully symmetric non bifurcating one)
   }
The $s_2$ symmetry precludes the \reqv\ from having a streamwise
traveling component and forces it to be spanwise traveling only.
At $\Reynolds = 400$, its velocity is very small,
$(c_x,c_z) = (0,0.00655)$.
  \JFG{
It would be good to illustrate this in more detail. I need more details myself.
Is there a change of stability associated with the production of \reqva, or
is it merely that an eigenfunction aligns with $\partial_x u$ and
$\partial_z u$ at some value of the bifurcation parameter? How do you
then construct an initial guess for the \reqv? Add $\bu$ and $\epsilon \times$
eigenfunction? I think a plot of alignment vs bifurcation parameter would be
helpful.
      }

\medskip
 These unstable
 flow-invariant solutions can only be computed numerically,
 but they are `exact' in the sense that they converge to
 solutions of the Navier-Stokes equations as the numerical resolution increases.


\medskip
Three \pCf\ \reqv\ solutions have been discussed in the literature.
The first two
were found by \cite{N97} by continuing \tLB\ to
a combined Couette / Poiseulle channel flow
then continuing back to \pCf.
The result is a pair of streamwise-traveling
\reqva\ connected by
a saddle-node bifurcation, similar to \tLB\ and \tUB.

